Trustworthy Reinforcement Learning Against Intrinsic Vulnerabilities: Robustness, Safety, and Generalizability

A trustworthy reinforcement learning algorithm should be competent in solving challenging real-world problems, including {robustly} handling uncertainties, satisfying {safety} constraints to avoid catastrophic failures, and {generalizing} to unseen scenarios during deployments. This study aims to overview these main perspectives of trustworthy reinforcement learning considering its intrinsic vulnerabilities on robustness, safety, and generalizability. In particular, we give rigorous formulations, categorize corresponding methodologies, and discuss benchmarks for each perspective. Moreover, we provide an outlook section to spur promising future directions with a brief discussion on extrinsic vulnerabilities considering human feedback. We hope this survey could bring together separate threads of studies together in a unified framework and promote the trustworthiness of reinforcement learning.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> figures/tree_overall.tex <==
% VERSION 3.0
\usetikzlibrary{trees}
\begin{tikzpicture}[
    % train/.style={fill=red!5,draw=red!50,draw},
    % both/.style={fill=red!50},
    i/.style={
        anchor=north,% south,
        align=center,
        top color=white,
        bottom color=blue!10,
        rectangle,rounded corners,
        minimum height=6mm,
        draw=blue!75,
        % very thick,
        align=center,
        color=blue!75,
        text=black,
        % font=\bfseries,
        text depth = 0pt
    }
]
    \tikzset{execute at begin node=\strut}
    \tikzset{font=\small,
        grow=down,
        % edge from parent fork right,
        level distance=1.5cm,
        every tree node/.style={align=center,anchor=north},
        every leaf node/.style=
            {
                anchor=north,% south,
                align=center,
                fill=blue!5,
                rectangle,
                % minimum height=8mm,
                draw=blue!50,
                % thick,
                align=center,
                distance=1cm,
                text depth = -10pt
            },
        edge from parent/.style=
            {
                draw=blue!50,
                thick,
                edge from parent path={(\tikzparentnode.south)
                -- +(0,-8pt)
                -| (\tikzchildnode)}
            }
    }
    
    
    
    \Tree [.\node[i] {Trustworthy RL};
    [
        .\node[i] {Robustness \treesec{(\S \ref*{sec:robust})}};
        [
        	.\node[i] {Individual components};
		    [
		        .\node[i] {Observation Space \treesec{(\S \ref*{sec:robust-ob})}};
		        [
		            .\node[i] {(Adversarial) \\Re-training};
		            {
		                \cite{behzadan2017whatever}
		                \cite{kos2017delving} \\
		                \cite{pattanaik2018robust}
		                \cite{gleave2019adversarial} \\
		                \cite{zhang2021atla}
		                \cite{sun2021strongest}
		            }
		        ]
		        [
		            .\node[i] {Regularizer};
		            {
		                \cite{zhang2021robust}
		                \cite{shen2020deep}
		            }
		        ]
		        [
		            .\node[i] {Worst-case \\Bounds};
		            {
		                \cite{everett2021certifiable}
		                \cite{oikarinen2020robust}
		            }
		        ]
		        [
		            .\node[i] {Detection\\ of\\ Adversary};
		            {
		                \cite{lin2017detecting}
		                \cite{havens2018online}
		            }
		        ]        
		    ]
		    [
		        .\node[i] {Environmental \\Dynamics
		        \treesec{(\S \ref*{sec:robust-env})}};
		        [
		            .\node[i] {Ensemble \\Learning};
		            {
		                \cite{rajeswaran2016epopt}
		            }
		        ]
		        [
		            .\node[i] {Adversarial \\Learning};
		            {
		                \cite{pinto2017robust}
		                \cite{mandlekar2017adversarially}
		            }
		        ]
		    ]
		    [
		        .\node[i] {Action Space \treesec{(\S \ref*{sec:robust-act})}};
		        [
		            .\node[i] {PR-MDP \\\& \\NR-MDP}; {
		                \cite{tessler2019action}
		            }
		        ]
		        [
		            .\node[i] {Real-Time \\RL}; {
		                \cite{hester2013texplore}
		                \cite{ramstedt2019real}\\
		                \cite{Xiao2020Thinking}
		            }
		        ]
		        [
		            .\node[i]{Action \\Delay}; {
		                \cite{schuitema2010control}
		                \cite{firoiu2018human}\\
		                \cite{bouteiller2021reinforcement}
		                \cite{chen2020delay}\\
		                \cite{chen2021delay} 
		            }
		        ]
		    ]
		    [
		        .\node[i] {Reward \treesec{(\S \ref*{sec:robust-reward})}};
		        [
		            .\node[i] {Reward \\Estimation \\ /Learning};
		            {
		                \cite{wang2020reinforcement}
		                \cite{romoff2018reward}\\
		                \cite{fu2017learning}
		            }
		        ]
		        [
		            .\node[i] {Region \\Based};
		            {
		                \cite{huang2019deceptive}
		                \cite{zhang2020adaptive}
		            }
		        ]
		        [
		            .\node[i] {Others};
		            {
		                \cite{zhang2021robustpg}
		                \cite{talvitie2018learning}
		            }
		        ]
		    ]
        ]
        [
        	.\node[i] {Distributionally robust RL};
		    [
		        .\node[i]{Uncertainty dist. \\
		        as transition dist and reward function};
		        {
		            \cite{abdullah2019wasserstein, 
		                    sinha2017certifying,
		                    lecarpentier2019non,
		                    mankowitz2019robust,
		                    smirnova2019distributionally}
		        }
		    ]
		    [
		        .\node[i]{Uncertainty parameter \\
		        as transition dist and reward function};
		        [
		            .\node[i] {MDP};
		            [
		                .\node[i] {Discrepancy-based \\
		                uncertainty set};
		                {
		                    % todo: citations
		                    \cite{yang2017convex,
		                    osogami2012robustness,
		                    chen2019distributionally,
		                    derman2020distributional}
		                }
		            ]
		            [
		            .\node[i] {Moment-based\\
		            uncertainty set};
		            {
		                % todo: citations
		                \cite{xu2010distributionally,
		                abdullah2019wasserstein,
		                chen2019distributionally}
		            }
		        ]
		        ]
		        [
		        .\node[i] {POMDP};
		        {
		            % todo: citations
		            \cite{nakao2021distributionally}
		        }
		        ]
		    ]
		    [
		        .\node[i]{Discussion};
		        [
		            .\node[i] {Game theory};
		            [
		                .\node[i] {Robust game};
		                {
		                    % todo: citations
		                    \cite{aghassi2006robust}
		                }
		            ]
		            [
		                .\node[i] {Distributionally \\
		                robust game};
		                {
		                    % todo: citations
		                    \cite{sengupta2020multi}
		                    \cite{liu2018distributionally}
		                }
		            ]
		        ]
		        [
		            .\node[i] {Time (in)consistency \\
		            for multistage DRO};
		            {
		                 % todo: citations
		                 \cite{xin2021time, shapiro2021tutorial}
		            }
		        ]
		        [
		            .\node[i] {Choices of \\
		            uncertainty set};
		            {
		                 % todo: citations
		                 \cite{smirnova2019distributionally}
		            }
		        ]
		    ]
        ]
    ]
    [
        .\node[i] {Safe learning
         \treesec{(\S \ref*{sec:safe})}};
	    [
	        .\node[i] {Lagrangian};
	        [
	            .\node[i]{Manual Selection of\\Lagrange Multiplier};
	            {
	                \cite{borkar2005actor}
	                \cite{bhatnagar2012online}
	            }
	        ]
	        [
	            .\node[i]{Primal-dual};
	            {
	                \cite{chow2017risk}
	                \cite{achiam2017constrained}
	                \cite{liang2018accelerated}
	                \cite{tessler2018reward}
	                \\
	                \cite{paternain2019constrained}
	                \cite{stooke2020responsive}
	                \cite{yu2019convergent}
	            }
	        ]
	        [
	            .\node[i] {Projection};
	            {
	                \cite{zhang2020first}
	                \cite{yang2020projection}
	                \\
	                \cite{yang2021accelerating}
	            }
	        ]
	    ]
	    [
	        .\node[i] {Uncertainty-aware};
	        [
	            .\node[i] {UCB};
	            {
	                \cite{singh2020learning}
	                \cite{efroni2020exploration}
	                \\
	                \cite{brantley2020constrained}
	                \cite{ding2021provably}
	            }
	        ]
	        [
	            .\node[i] {dynamics \\ uncertainty};
	            {
	                \cite{koller2018learning}
	                \cite{thananjeyan2020safety}
	                \\
	                \cite{liu2020constrained}
	                \cite{chen2021context}
	            }
	        ]
	    ]
	    [
	        .\node[i] {Leveraging the\\Prior Knowledge};
	        [
	            .\node[i] {Lyapunov};
	            {
	                \citep{berkenkamp2017safe}
	                \citep{richards2018lyapunov}
	                \citep{chow2019lyapunov}
	            }
	        ]
	        [
	            .\node[i] {Control barrier \\ functions};
	            {
	                \citep{li2019temporal}
	                \citep{cheng2019end}
	            }
	        ]
	        [
	            .\node[i] {Post-process\\Safety Layer};
	            {
	                \cite{pham2018optlayer}
	                \cite{dalal2018safe}
	            }
	        ]
	        [
	            .\node[i] {Formal \\ Verification};
	            {
	                \cite{li2019temporal}
	                \cite{liu2021recurrent}
	                \cite{puranic2021learning}
	            }
	        ]
	    ]
	    [
	        .\node[i] {Others};
	            {
	                \cite{mehta2020curriculum}
	                \cite{srinivasan2020learning}
	                \cite{turchetta2020safe}
	                \cite{thananjeyan2021recovery}
	            }
	    ]
    ]
    [
        .\node[i] {Generalization to \\OOD distribution
         \treesec{(\S \ref*{sec:generalization})}};
        {
            Sim2Real RL\\
            Adaptation to nonstationary environment\\
            Resilience to sparsity
        }
    ]
    [
        .\node[i] {Interpretable RL
         \treesec{(\S \ref*{sec:interpretable})}};
        [
            .\node[i] {Feature-based \\ \treesec{(\S \ref*{sec:interpret-feature})}};
            {
                TBD
            }
        ]
        [
            .\node[i] {Structure-based \\ \treesec{(\S \ref*{sec:interpret-structure})}};
            {
                TBD
            }
        ]
        [
            .\node[i] {Knowledge-based \\ \treesec{(\S \ref*{sec:interpret-knowledge})}};
            [
                .\node[i] {Neuro-symbolic \\ Action Space};
                {
                    \cite{ma2021learning}
                    \cite{garnelo2016towards} 
                    \cite{lyu2019sdrl} \\
                    \cite{xu2021interpretable} 
                    \cite{anderson2020neurosymbolic}
                    \cite{lyu2021tdm} \\
                    \cite{verma2018programmatically}
                    \cite{hein2018interpretable}
                    \cite{maes2012policy} \\
                    \cite{verma2019verifiable}
                    \cite{penkov2019learning}
                    \cite{lange2019semantic} \\
                    \cite{christodoulou2019reinforcement}
                    \cite{bastani2018verifiable}
                    \cite{silva2020optimization}
                }
            ]
            [
                .\node[i] {External Knowledge \\ Guided Training};
                {
                    \cite{bougie2020towards}
                    \cite{argerich2020tutor4rl}
                    \cite{cheng2021heuristic} \\
                    \cite{garcez2018towards}
                    \cite{juozapaitis2019explainable}
                    \cite{sheikh2020learning}
                }
            ]
            [
                .\node[i] {Post-hoc \\ Explanation};
                {
                    \cite{frosst2017distilling}
                    \cite{liu2018toward}
                    \cite{sun2020cracking} \\
                    \cite{dhebar2020interpretable}
                    \cite{vasic2019moet}
                    \cite{ding2020cdt} \\
                    \cite{deletang2021causal}
                    \cite{madumal2020explainable}
                }
            ]
        ]
    ]
    [
        .\node[i] {Building trust \\with human
         \treesec{(\S \ref*{sec:trust})}};
        {
            Understanding the human\\
            Privacy in RL\\
            Fairness in RL
        }
    ]
    [
        .\node[i] {Evaluation and \\verification for RL
         \treesec{(\S \ref*{sec:evaluation})}};
        {
            Evaluation\\
            Certification
        }
    ]
    ]
\end{tikzpicture}

% \begin{tikzpicture}[grow'=right,level distance=1.25in,sibling distance=.25in]
% \tikzset{edge from parent/.style= 
%             {thick, draw, edge from parent fork right},
%          every tree node/.style=
%             {draw,minimum width=1in,text width=1in,align=center}}
% \Tree 
%     [. parent 
%         [.{nice child0}
%                 [.{grandchild0-0 } ]
%             [.{grandchild0-1 } ]
%             [.{grandchild0-2 } ]
%             [.{grandchild0-3 } ]
%         ]
%         [.child1
%                 [.{grandchild1-0 } ]
%             [.{grandchild1-1 } ]
%             [.{grandchild1-2 } ]
%         ] 
%         [.child2 ]
%         [.child3 ]
%     ]
% \end{tikzpicture}

% \bibliographystyle{plainnat}
% \bibliography{ref}
% \end{document}

==> papers.tex <==
\noindent\underline{\Large Survey papers}:

\vspace{2em}
\href{https://cmp.felk.cvut.cz/~peckama2/papers/safe_exploration_overview_lncs.pdf}{Safe exploration techniques for reinforcement learning an overview}~\cite{pecka2014safe}

\vspace{2em}
\href{https://jmlr.org/papers/v16/garcia15a.html}{A Comprehensive Survey on Safe Reinforcement Learning
}~\cite{garcia2015comprehensive}

\vspace{2em}
\href{https://arxiv.org/abs/1606.06565}{Concrete Problems in AI Safety}~\cite{amodei2016concrete}

\textbf{Accidents: }
unintended and harmful behavior that may emerge from poor design of real-world AI systems, 
\begin{itemize}[noitemsep,nolistsep]
    \item wrong objective functions ("negative side effect", "reward hacking")
    \item the correct objective function too expensive to evaluate, leading to bad extrapolations from limited samples ("scalable oversight")
    \item insufficient or poorly curated training data or an insufficiently expressive model ("safe exploration", "distributional shift")
\end{itemize}

\vspace{2em}
\href{https://arxiv.org/pdf/1602.03506.pdf}{Research Priorities for Robust and Beneficial Artificial Intelligence}~\cite{russell2015research}


short-term
\begin{itemize}[noitemsep,nolistsep]
    \item \textbf{Verification: }(``Did I build the system right?'')
    
    \begin{itemize}[noitemsep,nolistsep]
        \item verify the designs of the AI systems themselves, particularly if they follow a ``componentized architecture'' / distinct modules (predictive models, state estimates, utility functions, policies, learning elements, etc.)
        \item differences compared with traditional software verification: 
        1) Agents operate in \textit{environments} that are at best \textit{partially known} by the system designer;
        2) A lack of design-time knowledge also motivates the use of learning algorithms within the agent software, and veriﬁcation becomes more diﬃcult
    \end{itemize}
    
    \item \textbf{Validity: }(``Did I build the right system?'')
    \begin{itemize}[noitemsep,nolistsep]
        \item ubiquitous specification errors in software verificatons; the notions of “beneﬁcial” and “desirable” are not formal
        \item computational expense of diﬀerent behavioral standards (or ethical theories)
    \end{itemize}
    
    \item \textbf{Security: }(how to prevent intentional manipulation by unauthorized parties.)
    
    \item \textbf{Control: }(``OK, I built the system wrong; can I ﬁx it?'')
    \begin{itemize}[noitemsep,nolistsep]
        \item retain some form of meaningful human control
        \item The design of systems and protocols for transition between automated navigation and human control; how to optimally allocate tasks within human–computer teams
    \end{itemize}
    
\end{itemize}


long-term

\vspace{2em}
\href{https://arxiv.org/pdf/1711.09883.pdf}{AI Safety Gridworlds}~\cite{leike2017ai}

a test suite for safety problems

each environment equipped with a reward function $R$ and a (safety) performance function $R^\star$
\begin{itemize}[noitemsep,nolistsep]
    \item specification problem: $R\neq R^\star$ [Safe interruptibility, Avoiding side effects, Absent supervisor, Reward gaming]
    \item robustness problem: $R=R^\star$ [Self-modiﬁcation, Distributional shift, Robustness to adversaries, Safe exploration]
\end{itemize}

\textbf{Exp:} A2C and Rainbow on all these environments

\textbf{Conclusions:} they struggle with achieving the maximal return in the \textit{robustness problems}, and they do not perform well according to the \textit{speciﬁcation environments}’ performance functions

\textbf{Discussions:}

- solutions that generalize: involve general heuristics; humans in the loop

- one way to alleviate the specifications problem: reward learning, train a reward predictor to learn a reward function corresponding to the performance function

\vspace{2em}
\href{https://arxiv.org/pdf/1610.03295.pdf}{Safe, Multi-Agent, Reinforcement Learning for Autonomous Driving}~\cite{shalev2016safe}


\vspace{4em}
\noindent\underline{\Large Safe exploration}

\vspace{2em}
\href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.161.2786&rep=rep1&type=pdf}{Safe Exploration for Reinforcement Learning}~\cite{hans2008safe}

\vspace{2em}
\href{https://scholar.google.com/scholar_url?url=https://www.jair.org/index.php/jair/article/download/10789/25759&hl=en&sa=T&oi=gsb-gga&ct=res&cd=0&d=10252639304848426859&ei=QI-9YPu2EYWEywSIu7WQAg&scisig=AAGBfm0GMXuEvqY6Ev9AhVdhXBHvKxDaGg}{Safe Exploration of State and Action Spaces in Reinforcement Learning}~\cite{garcia2012safe}

\vspace{2em}
\href{https://arxiv.org/pdf/1705.08551.pdf}{Safe Model-based Reinforcement Learning with Stability Guarantees}~\cite{berkenkamp2017safe} [\href{https://youtu.be/Xwu38vQb9Gk}{youtube}]

from \textbf{control theory}

safety in terms of stability guarantees: \textbf{asymptotic stability} (ability to recover from exploratory actions)

starting from an initial, safe policy, we can 
\begin{itemize}[noitemsep,nolistsep]
    \item expand our estimate of the \textit{region of attraction} by collecting data inside the safe region
    \item adapt the policy to both increase the region of attraction and improve control performance.
\end{itemize}

\vspace{2em}
\href{https://arxiv.org/pdf/1803.08287.pdf}{Learning-based Model Predictive Control for Safe Exploration}~\cite{koller2018learning}

\vspace{2em}
\href{https://arxiv.org/pdf/1205.4810.pdf}{Safe Exploration in Markov Decision Processes}~\cite{moldovan2012safe}

\vspace{2em}
\href{https://arxiv.org/pdf/1606.04753.pdf}{Safe Exploration in Finite Markov Decision Processes
with Gaussian Processes}~\cite{turchetta2016safe}


\vspace{4em}
\noindent\underline{\Large Model predictive control}

\vspace{2em}
\href{https://arxiv.org/pdf/1107.2487.pdf}{Provably Safe and Robust Learning-Based Model Predictive Control}~\cite{aswani2013provably}

\vspace{2em}
\href{https://www2.eecs.berkeley.edu/Pubs/TechRpts/2015/EECS-2015-190.pdf}{Reachability-based Safe Learning with Gaussian Processes}~\cite{akametalu2014reachability}

\vspace{4em}
\noindent\underline{\Large Robust MDP}

\vspace{2em}
\href{http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.414.2814&rep=rep1&type=pdf}{Robust Markov Decision Processes}~\cite{wiesemann2013robust}

\vspace{2em}
\href{https://arxiv.org/pdf/1306.6189.pdf}{Scaling Up Robust MDPs by Reinforcement Learning}~\cite{tamar2013scaling}

\vspace{2em}
\href{https://scholar.google.com/scholar_url?url=https://www.jair.org/index.php/jair/article/download/10415/24966/&hl=en&sa=T&oi=gsb-gga&ct=res&cd=0&d=7363114586501816208&ei=-d68YPibHJj0yATT4byYCg&scisig=AAGBfm3byP2MH2UwRvNKmH7PAs80Z-D6Kw}{Risk-Sensitive Reinforcement Learning Applied to Control under Constraints}~\cite{geibel2005risk}

\vspace{4em}
\noindent\underline{\Large Safe policy search methods}

\vspace{2em}
\href{http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.1059.1383&rep=rep1&type=pdf}{Constrained Reinforcement Learning from
Intrinsic and Extrinsic Rewards}~\cite{uchibe2007constrained}
 
\vspace{2em}
\href{http://proceedings.mlr.press/v37/ammar15.pdf}{Safe Policy Search for Lifelong Reinforcement Learning with Sublinear Regret}~\cite{ammar2015safe}

\vspace{2em}
\href{https://www.jmlr.org/papers/volume18/15-636/15-636.pdf}{Risk-Constrained Reinforcement Learning with Percentile Risk Criteria}~\cite{chow2017risk}

\vspace{2em}
\href{https://arxiv.org/pdf/1705.05394.pdf}{Probabilistically Safe Policy Transfer}~\cite{held2017probabilistically}

\vspace{2em}
\href{https://arxiv.org/pdf/1705.10528.pdf}{Constrained Policy Optimization}~\cite{achiam2017constrained}

the ﬁrst general-purpose policy search algorithm for constrained reinforcement learning with guarantees for near-constraint satisfaction at each iteration.

\textbf{problem setup: }
MDP with a set $C$ of auxiliary cost functions, $C_1,\ldots,C_m$ (with each one a function $C_i:S\times A\times S\rightarrow \bb R$) and cost function $J_{C_{i}}(\pi)=\mathrm{E}\left[\sum_{t=0}^{\infty} \gamma^{t} C_{i}\left(s_{t}, a_{t}, s_{t+1}\right)\right]$.

\textbf{constrained policy update:}
\begin{align*}
\pi_{k+1}=\arg \max _{\pi \in \Pi_{\theta}} & J(\pi) \\
\text { s.t. }& {\color{red} J_{C_{i}}(\pi) \leq d_{i} \quad i=1, \ldots, m} \\
& D\left(\pi, \pi_{k}\right) \leq \delta .
\end{align*}

\textbf{policy performance bounds:}
\begin{align*}
J\left(\pi^{\prime}\right)-J(\pi) 
\geq \frac{1}{1-\gamma} \underset{a \sim \pi^{\prime}}{\mathrm{E}}\left[A^{\pi}(s, a)-\frac{2 \gamma \epsilon^{\pi^{\prime}}}{1-\gamma} D_{T V}\left(\pi^{\prime} \| \pi\right)[s]\right]
\end{align*}

plus \textbf{trust region methods:}
\begin{align*}
\pi_{k+1}=& \arg \max _{\pi \in \Pi_{\theta}} \underset{s \sim d^{\pi_{k}} \atop a \sim \pi}{\mathrm{E}}\left[A^{\pi_{k}}(s, a)\right] \\
\text { s.t. } & J_{C_{i}}\left(\pi_{k}\right)+\frac{1}{1-\gamma} \underset{s \sim d^{\pi_{k}}}{\mathrm{E}}\left[A_{C_{i}}^{\pi_{k}}(s, a)\right] \leq d_{i} \quad \forall i \\
& \bar{D}_{K L}\left(\pi \| \pi_{k}\right) \leq \delta .
\end{align*}


\vspace{2em}
\href{https://arxiv.org/pdf/1805.11074.pdf}{Reward Constrained Policy Optimization}~\cite{tessler2018reward}



\vspace{4em}
\noindent\underline{\Large Intersection with other disciplines}

\vspace{2em}
\href{https://www.pnas.org/content/pnas/116/50/24972.full.pdf}{Social behavior for autonomous vehicles}~\cite{schwarting2019social}

\textbf{Goal: }understand the intent of the human drivers and respond in a predictable and interpretable way.

\textbf{Steps:}

1. estimating SVO (Social Value Orientation) online from observed driving trajectories

\begin{figure}[h]
    \centering
    \includegraphics[width=.35\textwidth]{figures/fig_svo.png}
    \caption{\small SVO value}
    \label{fig:svo}
\end{figure}


2. integrating SVO preferences into the utility-maximizing framework:
\begin{align*}
G_{i}\left(\mathbf{x}^{0}, \mathbf{u}, \varphi_{i}\right)=\sum_{k=0}^{N-1} g_{i}\left(\mathbf{x}^{k}, \mathbf{u}^{k}, \varphi_{i}\right)+g_{i}^{N}\left(\mathbf{x}^{N}, \varphi_{i}\right)    
\end{align*}

3. modeling interactions between agents as a best-response game, compute a Nash equilibrium of the game defined below:
\begin{align*}
\mathbf{u}_{i}^{*}\left(\mathbf{x}^{0}, \varphi_{i}\right)=\underset{\mathbf{u}_{i}}{\arg \max } G_{i}\left(\mathbf{x}^{0}, \mathbf{u}_{i}, \mathbf{u}_{\neg i}, \varphi_{i}\right),
\end{align*}
corresponding to the actions maximizing the likelihood under the maximum entropy model
\begin{align*}
    P\left(\mathbf{u}_{i} \mid \mathbf{x}^{0}, \mathbf{u}_{\neg i}, \varphi_{i}\right) \propto \exp \left(G_{i}\left(\mathbf{x}^{0}, \mathbf{u}_{i}, \mathbf{u}_{\neg i}, \varphi_{i}\right)\right).
\end{align*}

\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{figures/fig_svo_algo.png}
    \caption{\small algo}
    \label{fig:svo-algo}
\end{figure}

\textbf{Conclusions: }
robotic and artiﬁcial intelligence applications where an autonomous system acts among humans will beneﬁt from integrating SVO in their prediction and decision-making algorithms.



==> symbol_table.tex <==
\section{Notation System}
\label{append:notations}

  \subsection{Notation Convention}
  \begin{enumerate}
    \item Function: lowercase letter, e.g. $f$, $f(\cdot)$ 
    \item Scalar: lowercase letter, e.g. $x$
    \item Random variable: uppercase letter, e.g. $X$
    \item Matrix:  uppercase letter, e.g. $K$
    \item Common number set: Upper case double letter, e.g. $\mathbb R$ 
    \item Context-based set: Upper case script letter, e.g. $\mathcal A$ 
  \end{enumerate}
  
  \subsection{Alphabet Letter}
  %\begin{table}[h!]
  
  \ding{rerank them by alphabetical order}
  \begin{longtable}{ |l|p{6cm}|p{6cm}|  }
     %\hline
     %\multicolumn{3}{|c|}{Alphabet Letter} \\
     \hline
     Symbol& Designation &Note/Example\\
     \hline
     %%%----- alphabet letters ------
     $\mathbb{1} (\cdot)$   & Indicator function    & \\
     \hline
      $d $   & dimension of input variable   & \\
     \hline
     $\mathcal D$   & dataset   & \\
     \hline
     $\mathbb E[\cdot]$   & Expectation    & -\\
     \hline
     $\mathbb E_p [\cdot]$   & Expectation taken with pdf $p$    & -\\
     \hline
      $f, f (\cdot)$   & Mapping representation of system, relating input to output  & \\
       \hline
         $\mathcal{GP}(m, K) $   & Gaussian process with mean $m$ and covariance $K$    & \\
     \hline
     $n$   & Number of samples    & \\
     \hline
     $\mathcal{N}(\mu, \sigma^2I) $   & Normal distribution with mean $\mu$ and variance $\sigma^2$    & \\
     \hline
     $p$   & Probability distribution (original)    & \\
     \hline
     $P (\cdot)$   & Probability    & \\
     \hline
     $q$   & Probability distribution (biasing/proposal)    & \\
     \hline
     $\mathcal Q$   & Set of proposal distributions    & \\
     \hline
     $\mathbb{R} $   & Real set    & \\
     \hline
     $\text{Std}(\cdot) $   & Standard Deviation    & \\
     \hline
     $\text{Var}(\cdot) $   & Variance    & \\
     \hline
     $x$   & A generic variable representing input to system & The default is $x = [x_1, \cdots, x_d]$ \\
     \hline
     $X$   & Random variable representation of $x$ & $X^{(1)}, \cdots, X^{(n)}$ means $n$ samples of $X$. Each sample $X^{(i)} = [X_1^{(i)}, \cdots, X_d^{(i)}]$, for $i=1, 2, \cdots, n$. \\
     \hline
     $y$   & Variable representing output of the system    & $y = f(x)$\\
     \hline
     $Y$   & Random variable representation of $y$    & $Y = f(X)$\\
     \hline
     $s$   & a state    & \\
     \hline
      $s^\prime$   & the next state    & \\
     \hline
     $\mathcal{S}$   & state space    & $s \in \mathcal{S}$\\
     \hline 
     $a$   & an action   & \\
     \hline
     $\mathcal{A}$   & action space    & $a \in \mathcal{A}$\\
     \hline 
      $r(s,a)$   & expected immediate reward from state $s$ after action $a$    & \\
     \hline
     $G_t$   & return (discounted cumulative reward) following time t  & $G = \sum_{t} \gamma^t r_t $\\
     \hline 
      $p(s^\prime | s, a)$   & probability of transition to state $s^\prime$, from state $s$ taking action $a$  &\\
     \hline 
       $J(\theta)$   & performance measure for the policy $\pi_\theta$  &\\
     \hline
      $L$   & loss function  &\\
      
     \hline
     
    \end{longtable}
    %\end{table}
  
  \subsection{Greek Letter}
  \begin{table}[h!]
      \begin{tabular}{ |l|p{6cm}|p{6cm}|  }
     \hline
     Symbol& Designation &Note/Example\\
     \hline
     %%%----- greek letters ------
     $\epsilon$   & Small positive scalar   & (epsilon or varepsilon)\\
     \hline
     $\theta$   & Parameter of system approximation & -\\
     \hline
      $\Theta$   & Set of possible parameters & $\theta \in \Theta$\\
     \hline
     $\mu$   & Mean & -\\
     \hline
     $\mu_X$   & Mean of random variable $X$   & -\\
     \hline
     $\sigma$   & (Unbiased) standard deviation   & $\sigma^2$: (Unbiased) Variance\\
     \hline
      $\sigma_X$   & (Unbiased) standard deviation of r.v. $X$ & $\sigma_X^2$: (Unbiased) variance of $X$\\
     \hline
      $\gamma$   & discount factor of reward & $R = \sum_{t} \gamma^t r_t $\\
     \hline
        $\tau$   & experience of an episode & $\tau = \{s_0, a_0, \dots, s_T, a_T \} $\\
     \hline
    $\pi$   & policy of an agent & $\pi(a | s)$: stochastic policy ; $\pi(s)$: deterministic policy\\
     \hline
    \end{tabular}
    \end{table}
